Categorification of the Jones-Wenzl Projectors

The Jones-Wenzl projectors play a central role in quantum topology, underlying the construction of SU(2) topological quantum field theories and quantum spin networks. We construct chain complexes whose graded Euler characteristic is the "classical" projector in the Temperley-Lieb algebra. We show that they are homotopy idempotents and uniquely defined up to homotopy. Our results fit within the general framework of Khovanov's categorification of the Jones polynomial. Consequences of our construction include families of knot invariants corresponding to higher representations of quantum su(2) and a categorification of quantum spin networks. We introduce 6j-symbols in this context.

==> graphicx.tex <==
% Plain TeX interface to graphicx package.
% David Carlisle


%\input miniltx

%\def\Gin@driver{dvips.def}
%\input graphicx.sty


%\resetatcatcode

\input miniltx

\ifx\pdfoutput\undefined
  \def\Gin@driver{dvips.def} % we are not running PDFTeX
\else
  \def\Gin@driver{pdftex.def} % we are running PDFTeX
\fi
 
\input graphicx.sty
\resetatcatcode


==> joneswenzl final arxiv/graphicx.tex <==
% Plain TeX interface to graphicx package.
% David Carlisle


%\input miniltx

%\def\Gin@driver{dvips.def}
%\input graphicx.sty


%\resetatcatcode

\input miniltx

\ifx\pdfoutput\undefined
  \def\Gin@driver{dvips.def} % we are not running PDFTeX
\else
  \def\Gin@driver{pdftex.def} % we are running PDFTeX
\fi
 
\input graphicx.sty
\resetatcatcode

